Class-Imbalanced Learning on Graphs: A Survey

The rapid advancement in data-driven research has increased the demand for effective graph data analysis. However, real-world data often exhibits class imbalance, leading to poor performance of machine learning models. To overcome this challenge, class-imbalanced learning on graphs (CILG) has emerged as a promising solution that combines the strengths of graph representation learning and class-imbalanced learning. In recent years, significant progress has been made in CILG. Anticipating that such a trend will continue, this survey aims to offer a comprehensive understanding of the current state-of-the-art in CILG and provide insights for future research directions. Concerning the former, we introduce the first taxonomy of existing work and its connection to existing imbalanced learning literature. Concerning the latter, we critically analyze recent work in CILG and discuss urgent lines of inquiry within the topic. Moreover, we provide a continuously maintained reading list of papers and code at https://github.com/yihongma/CILG-Papers.

==> tables/confusion.tex <==
\begin{table}[t]
\captionsetup{width=0.6\textwidth}
\caption{Confusion matrix for a binary classification problem.}
\label{tab:confusion}
\begin{center}
\resizebox{0.6\textwidth}{!}
{\begin{NiceTabular}{ccc}
\toprule
& Positive Prediction & Negative Prediction \\
\midrule
Positive Class & True Positive (TP) & False Negative (FN) \\
Negative Class & False Positive (FP) & True Negative (TN) \\
\bottomrule
\end{NiceTabular}}
\end{center}
\end{table}

==> tables/metrics.tex <==
% \begin{table}[t]
% \begin{center}
% \captionsetup{width=.55\textwidth}
% \caption{A comprehensive overview of evaluation metrics for node classification tasks, including their formulas and suitability for use in the context of CILG methods.}
% \label{tab:metrics}
% \resizebox{0.55\textwidth}{!}
% {\begin{NiceTabular}{c|c|c}[]
% \toprule
% \textbf{Metric} & \textbf{Formula} & \textbf{CILG}\\ 
% \midrule
% Sensitivity & $\cfrac{\text{TP}}{\text{TP} + \text{FN}}$ & \ding{51} \\
% \midrule
% Specificity & $\cfrac{\text{TN}}{\text{TN} + \text{FP}}$ & \ding{55} \\
% \midrule
% Precision & $\cfrac{\text{TP}}{\text{TP} + \text{FP}}$ & \ding{51} \\
% \midrule
% Recall & $\cfrac{\text{TP}}{\text{TP} + \text{FN}}$ & \ding{51} \\
% \midrule
% Accuracy & $\cfrac{\text{TP}}{\text{TP} + \text{TN} + \text{FP} + \text{FN}}$ & \ding{55} \\
% \midrule
% bal. Accuracy & $\cfrac{\text{sensitivity} + \text{specificity}}{2}$ & \ding{51} \\
% \midrule
% G-Mean & $\sqrt{\text{sensitivity} \cdot \text{specificity}}$ & \ding{51} \\
% \midrule
% F-Measure & $\cfrac{2 \cdot \text{precision} \cdot \text{recall}}{\text{precision} + \text{recall}}$ & \ding{51} \\
% \midrule
% AUC-ROC & - & \ding{51} \\
% \bottomrule
% \end{NiceTabular}}
% \end{center}
% \end{table}

\begin{table}[t]
\captionsetup{width=0.8\textwidth}
\caption{A summary of evaluation metrics used in studies on CILG methods.}
\label{tab:metrics-models}
\begin{center}
\resizebox{0.8\textwidth}{!}
{\begin{NiceTabular}{c|cccccccc}
\toprule
\multirow{2.4}{*}{\textbf{Model}} & \multicolumn{7}{c}{\textbf{Evaluation Metrics}} \\ 
\cmidrule{2-9}
& \textbf{Acc} & \textbf{bAcc} & \textbf{GM} & \textbf{Prec} & \textbf{Recall} & \textbf{F$_\beta$} & \textbf{AUC} &\textbf{MCC} \\
\midrule
SPARC & \ding{51} & & & & \ding{51} & & \\
GraphSMOTE \cite{zhao2021graphsmote} & \ding{51} & & & & & \ding{51} & \ding{51} \\
GraphENS \cite{park2021graphens} & \ding{51} & \ding{51} & & & & \ding{51} & \\
ImGAGN \cite{qu2021imgagn} & & & & \ding{51} & \ding{51} & & \ding{51} \\
D-GCN \cite{wang2021dual} & & & & & & \ding{51} & \\
SET-GNN \cite{juan2021exploring} & \ding{51} & & & & & \ding{51} & \ding{51} \\
GraphMixup \cite{wu2022graphmixup} & \ding{51} & & & & & \ding{51} & \ding{51} \\
GATSMOTE \cite{liu2022gatsmote} & \ding{51} & & & & & \ding{51} & \ding{51} \\
SORAG \cite{duananonymity} & & & & & & \ding{51} & \\
DPGNN \cite{wang2022distance} & & & & & & \ding{51} & \\
GNN-CL \cite{li2022graph} & & & & & \ding{51} & & \ding{51} \\
GraphSR \cite{zhou2023graphsr} & \ding{51} & & & & & \ding{51} & \ding{51} \\
\midrule
RSDNE \cite{wang2018rsdne} & & & & & & \ding{51} & \\
ImVerde \cite{wu2018imverde} & \ding{51} & & & \ding{51} & & & \ding{51} \\
DR-GCN \cite{shi2020multi} & \ding{51} & & & & & & \ding{51} \\
RECT \cite{wang2020network} & & & & & & \ding{51} & \\
ReNode \cite{chen2021topology} & & & & & & \ding{51} & \\
FRAUDRE \cite{zhang2021fraudre} & & & & & \ding{51} & \ding{51} & \ding{51} \\
TAM \cite{song2022tam} & & \ding{51} & & & & \ding{51} & \\
CM-GCL \cite{qian2022comodality} & & & & & & \ding{51} & \ding{51} \\
LTE4G \cite{yun2022lte4g} & & \ding{51} & \ding{51} & & & \ding{51} & \\
ACS-GNN \cite{ma2022attention} & & & & & & \ding{51} & & \ding{51} \\
EGCN \cite{wang2022effective} & & & \ding{51} & & & \ding{51} & \ding{51} \\
KINC-GCN \cite{bai2022kernel} & \ding{51} & & & & & \ding{51} & \\
FACS-GCN \cite{santos2022facs} & & & & & \ding{51} & & \ding{51} \\
GraphDec \cite{zhang2022diving} & \ding{51} & \ding{51} & & & & \ding{51} & \\
ImGCL \cite{zeng2022imgcl} & \ding{51} & & & \ding{51} & \ding{51} & & \\
\bottomrule
\end{NiceTabular}}
\end{center}
\end{table}
